Bandlimited signal reconstruction from leaky integrate-and-fire encoding using POCS

Leaky integrate-and-fire (LIF) encoding is a model of neuron transfer function in biology that has recently attracted the attention of the signal processing and neuromorphic computing communities as a technique of event-based sampling for data acquisition. While LIF enables the implementation of analog-circuit signal samplers of lower complexity and higher accuracy simultaneously, the core difficulty of this technique is the retrieval of an input from its LIF-encoded output. In this article, we study this problem in the context of bandlimited inputs, by extracting the most abstract features of an LIF encoder as a generalized nonuniform sampler. In this view, the LIF output is seen as the transformation of the input by a known linear operator. We show that the signal reconstruction method of projection onto convex sets (POCS) converges to a weighted pseudo-inverse of this operator. This allows perfect recovery under uniqueness of reconstruction, minimum-norm reconstruction under incomplete sampling, as well as a noise shaping of time quantization that outperforms standard pseudo-inversion. On the practical side, a single iteration of the POCS method can be used to improve any estimate whose LIF samples are not consistent with those of the input, and a rigorous discrete-time implementation of this iteration is proposed that does not require a Nyquist-rate representation of the signals.

==> decl.tex <==
%\topmargin-0.5in

\usepackage{amssymb,amscd,bm}
%\usepackage{amssymb,amscd}
\usepackage[mathscr]{eucal}
%\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{enumitem}

\usepackage[usenames,dvipsnames]{pstricks}
\usepackage{epsfig}
\usepackage{pst-grad} % For gradients
\usepackage{pst-plot} % For axes

%-------------------------------- HYPERLINKS -----------------------------
\usepackage{srcltx}
\usepackage{xcolor}
\definecolor{dred}{rgb}{0.85,0.00,0.00}
\definecolor{dgreen}{rgb}{0.00,0.49,0.00}
\definecolor{dblue}{rgb}{0,0.08,1.00}
%\RequirePackage[bookmarks=false,dvipdfm,colorlinks,hyperindex]{hyperref}
\RequirePackage[bookmarks=false,driverfallback=dvipdfm,colorlinks,hyperindex]{hyperref}
%\RequirePackage[bookmarks=false,dvips,colorlinks,hyperindex]{hyperref}
% http://tug.ctan.org/cgi-bin/ctanPackageInformation.py?id=hyperref
\hypersetup{
    linktocpage=true,
    citecolor=dblue,    % color can be changed!
    linkcolor=dred    % color can be changed!
}

%\usepackage[pdftex,final]{graphicx}

\usepackage[T3,T1]{fontenc}

\DeclareSymbolFont{tipa}{T3}{cmr}{m}{n}
\DeclareMathAccent{\ib}{\mathalpha}{tipa}{16}


\def\TT{{\mathbb T}}
\def\RR{{\mathbb R}}
\def\ZZ{{\mathbb Z}}
\def\uu{\mathbb{1}}
\def\bZ{{\bf Z}}

\def\a{\mathrm{a}}
\def\b{\mathrm{b}}
\def\c{{\mathrm c}}
\def\d{\mathrm{d}}
\def\e{\mathrm{e}}
\def\f{\mathrm{f}}
\def\g{\mathrm{g}}
\def\h{\mathrm{h}}
\def\i{\mathrm{i}}
\def\q{\mathrm{q}}
\def\r{\mathrm{r}}
\def\p{{\bm p}}
\def\s{\mathrm{s}}
\def\t{{\bm t}}
\def\u{\mathrm{u}}
\def\v{\mathrm{v}}
\def\w{\mathrm{w}}
\def\x{{\bm x}}
\def\y{\mathrm{y}}
\def\z{\mathrm{z}}

\def\hA{\mathbf{\hat A}}
\def\hP{\mathbf{\hat P}}
\def\hQ{\mathbf{\hat Q}}
\def\hR{\mathbf{\hat R}}
\def\hT{\mathbf{\hat T}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\D{{\bm D}}
\def\H{{\mathbf H}}
\def\I{{\sf I}}
\def\J{{\sf J}}
\def\bM{{\mathbf M}}
\def\P{{\mathbf P}}
\def\Q{{\mathbf Q}}
\def\R{{\mathbf R}}
\def\T{{\mathbf T}}
\def\V{{\mathbf V}}
\def\W{{\mathbf W}}


\def\ca{{\bm a}}
\def\cp{{\bm p}}
\def\cq{{\bm q}}
\def\cs{{\bm s}}
\def\cu{{\bm u}}
\def\cv{{\bm v}}
\def\cx{{\bm x}}
\def\cy{{\bm y}}
\def\hca{\bm{\hat a}}

\def\balpha{{\bm\alpha}}
\def\bbeta{{\bm\beta}}
\def\blambda{{\bm\lambda}}
\def\btau{{\bm\tau}}
\def\btheta{{\bm\theta}}
\def\bhtheta{{\bm{\hat\theta}}}
\def\bbtheta{{\bm{\bar\theta}}}

\def\ba{{\bm a}}
\def\bb{{\bm b}}
\def\bc{{\bm c}}
\def\bd{{\bm d}}
\def\be{{\bm e}}
\def\bg{{\bm g}}
\def\bh{{\bm h}}
\def\bp{{\bm p}}
\def\br{{\bm r}}
\def\bs{{\bm s}}
\def\bq{{\bm q}}
\def\br{{\bm r}}
\def\bu{{\bm u}}
\def\bv{{\bm v}}
\def\bw{{\bm w}}
\def\bx{{\bm x}}
\def\by{{\bm y}}
\def\bz{{\bm z}}

\def\bdelta{{\bm\delta}}
\def\bzero{{\bf 0}}
\def\bone{{\bf 1}}

\def\K{{\sf K}}
\def\L{{\sf L}}
\def\N{{\sf N}}
\def\M{{\sf M}}
\def\Z{{\sf Z}}
\def\mod{\mathrm{mod}}
\def\sinc{\mathrm{sinc}}
\def\Si{\mathrm{Si}}
\def\Re{\mathrm{Re}}
\def\MSE{\mathrm{MSE}}
\def\sgn{\mathrm{sgn}}
\def\rel{\mathrm{relax}}
\def\msb{\mathrm{msb}}
\def\To{T_\mathrm{o}}
\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calC{{\cal C}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calG{{\cal G}}
\def\calH{{\cal H}}
\def\calI{{\cal I}}
\def\calJ{{\cal J}}
\def\calL{{\cal L}}
\def\calM{{\cal M}}
\def\calP{{\cal P}}
\def\calQ{{\cal Q}}
\def\calR{{\cal R}}
\def\calS{{\mathcal S}}
\def\calV{{\cal V}}
\def\calX{{\cal X}}
\def\calY{{\cal Y}}
\def\calZ{{\cal Z}}

\def\hcC{{\cal\hat C}}
\def\hcI{{\cal\hat I}}
\def\hcS{{\cal\hat S}}

\def\scA{{\mathscr A}}
\def\scB{{\mathscr B}}
\def\scC{{\mathscr C}}
\def\scH{{\mathscr H}}
\def\scG{{\mathscr G}}
\def\scL{{\mathscr L}}
\def\scP{{\mathscr P}}
\def\scR{{\mathscr R}}
\def\scS{{\mathscr S}}
\def\scV{{\mathscr V}}

\def\smallsum#1{{\textstyle\sum\limits_{#1}}}
\renewcommand{\smallint}[2]{{\textstyle\int\limits_{\raisebox{.1ex}{$\scriptstyle #1$}}^{\raisebox{.4ex}{$\scriptstyle #2$}}}}

\def\up#1{^{\scriptscriptstyle(#1)}}
\def\der#1{^{\scriptscriptstyle[#1]}}
%\renewcommand{\baselinestretch}{1.16}

\def\nN{_{n\in\N}}
\def\HS{\upsmall{\mathrm{HS}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{property}[theorem]{Property}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{result}[theorem]{Result}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{propdef}[theorem]{Proposition and Definition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}



\def\pp{\par\medskip}
\def\ppnoi{\par\medskip\noindent}
\def\line{\par\noindent}
\def\page{\vfill\eject}
\def\ccc{\centerline}

%++++++++++++++++++++++++++++++++++++++++++++++++++
\newcommand{\ZZS}{{\mathbb Z}^2}
\newcommand{\ZZP}{{\mathbb Z}^+}
\newcommand{\RRS}{{\mathbb R}^2}
\newcommand{\RRP}{{\mathbb R}^+}
\newcommand{\Exp}{{\mathbb E}}
\newcommand{\ZZnonz}{{\scrZ^*}}

\newcommand\figInclude[3]{
\begin{figure}
\centering
\graphicspath{{figure/}}
\includegraphics[totalheight=#1]{fig#2}
\caption{#3} \label{fig:#2}
\end{figure}
}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\comment}[1]{{\color{blue}[{\em #1}]}}

\newcommand{\dif}{{\mathrm d}}

\def\adc{\mbox{\small ADC}}
\def\dac{\mbox{\small DAC}}
\def\fft{\mathrm{FFT}}
\def\ran{\mathrm{ran}}
\def\rank{\mathrm{rank}}
\def\null{\mathrm{null}}
\def\var{\mathrm{Var}}


\def\mA{{\mathrm A}}
\def\mC{{\mathrm C}}
\def\mD{{\bf D}}
\def\mF{{\mathrm F}}
\def\mG{{\bf G}}
\def\mI{{\mathrm I}}
\def\mM{{\mathbf M}}
\def\mP{{\mathrm P}}
\def\mQ{{\mathrm Q}}
\def\mR{{\mathrm R}}
\def\mS{{\mathrm S}}
\def\mT{{\mathrm T}}
\def\mU{{\mathrm U}}
\def\mW{{\mathrm W}}
\def\mX{{\mathrm X}}
\def\mY{{\mathrm Y}}

\def\vA{{\mathrm A}}
\def\vI{{\mathrm I}}
\def\vM{{\mathrm M}}
\def\vR{{\mathrm R}}
\def\vS{{\mathrm S}}
\def\vT{{\mathrm T}}
\def\vU{{\mathrm U}}
\def\vV{{\mathrm V}}
\def\vX{{\mathrm X}}
\def\vY{{\mathrm Y}}


\def\va{{\mathbf a}}
\def\vb{{\mathbf b}}
\def\vc{{\mathbf c}}
\def\vd{{\mathbf d}}
\def\ve{{\mathbf e}}
\def\vf{{\mathbf f}}
\def\vg{{\mathbf g}}
\def\vh{{\mathbf h}}
\def\vi{{\mathbf i}}
\def\vj{{\mathbf j}}
\def\vm{{\mathbf m}}
\def\vx{{\mathbf x}}
\def\vy{{\mathbf y}}
\def\vo{{\mathbf o}}
\def\vp{{\mathbf p}}
\def\vq{{\mathbf q}}
\def\vr{{\mathbf r}}
\def\vs{{\mathbf s}}
\def\vt{{\mathbf t}}
\def\vu{{\mathbf u}}
\def\vv{{\mathbf v}}
\def\vw{{\mathbf w}}
\def\vz{{\mathbf z}}

\def\bvd{\mathbf{\bar d}}
\def\bve{\mathbf{\bar e}}
\def\hve{\mathbf{\hat e}}
\def\hvv{\mathbf{\hat v}}
\def\bvv{\mathbf{\bar v}}

\def\subin{\subsmall{\mathrm{in}}}
\def\subout{\subsmall{\mathrm{out}}}
\def\subP{\subsmall{\mathrm{P}}}
\def\subL{\subsmall{\mathrm{L}}}
\def\subC{\subsmall{\mathrm{C}}}

\def\ovl#1{{\overline{#1\!}\,}}
\def\sqrts#1{{\sqrt{#1\!}\,}}

\def\ssum#1{{\textstyle\sum\limits_{#1}}}
\def\sublow#1{_{_{\scriptstyle#1}}}
\def\subsmall#1{_{\scriptscriptstyle#1}}
\def\upsmall#1{^{\scriptscriptstyle#1}}
\def\eps{\epsilon}
\def\veps{\varepsilon}
\def\sinc{\mathrm{sinc}}
\def\sc{\mathrm{s}}

\newcommand{\half}{{\frac{1}{2}}}
\newcommand{\smallfrac}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\midfrac}[2]{\mbox{\footnotesize$\displaystyle\frac{#1}{#2}$}}
\newcommand{\smallhalf}{{\smallfrac{1}{2}}}

\def\subsmall#1{_{\scriptscriptstyle#1}}




